Privacy-Preserving Communication-Efficient Federated Multi-Armed Bandits

Communication bottleneck and data privacy are two critical concerns in federated multi-armed bandit (MAB) problems, such as situations in decision-making and recommendations of connected vehicles via wireless. In this paper, we design the privacy-preserving communication-efficient algorithm in such problems and study the interactions among privacy, communication and learning performance in terms of the regret. To be specific, we design privacy-preserving learning algorithms and communication protocols and derive the learning regret when networked private agents are performing online bandit learning in a master-worker, a decentralized and a hybrid structure. Our bandit learning algorithms are based on epoch-wise sub-optimal arm eliminations at each agent and agents exchange learning knowledge with the server/each other at the end of each epoch. Furthermore, we adopt the differential privacy (DP) approach to protect the data privacy at each agent when exchanging information; and we curtail communication costs by making less frequent communications with fewer agents participation. By analyzing the regret of our proposed algorithmic framework in the master-worker, decentralized and hybrid structures, we theoretically show tradeoffs between regret and communication costs/privacy. Finally, we empirically show these trade-offs which are consistent with our theoretical analysis.

==> Experiment.tex <==
\section{Simulations}

In this section, we conduct experiments to empirically verify the theoretical results of previous sections, that is, the trade-offs between communication, privacy and learning regret under different communication protocols. We first illustrate the simulation settings of our FMAB instances. There are $M=50$ agents, playing a MAB with Bernoulli rewards with 50 arms and randomly generated mean values. We show the experimental results of CDP-MAB (Alg. 1), DDP-MAB (Alg. 2) and HDP-MAB (Alg. 3) in the following. All algorithms were are run 50 times. 

\subsection{Centralized setting}

\subsubsection{Effect of Privacy Level $\epsilon$}
In this part, we allow all agents to communicate with the server at each communication rounds with a fixing the participating rate $p=1$ and only investigate the effect of privacy level $\epsilon$. We consider 4 different privacy parameters $\epsilon = \{0.3,0.5,0.7,1\}$. Fig. \ref{fig:epsilon} shows that the regret increases with the decreasing of  $\epsilon$ (higher level of privacy), since larger noises are added on the local update estimations. In particular, $\epsilon=1$ indicates the non-private case, in which we achieve about $5\times 10^4$ total regrets and the per-agent regret is around $1\times 10^3$.
\begin{figure}[h]
	\centering
	\includegraphics[width=0.6\linewidth]{../figures/epsilon}
	\caption{Regrets of CDP-MAB with different privacy level $\epsilon$.}
	\label{fig:epsilon}
\end{figure}

\begin{figure}[htbp]
	\centering
	\begin{minipage}[t]{1\textwidth}
		\centering
		\includegraphics[width=12cm]{../figures/prob_full}
		\caption{Regrets of CDP-MAB with different participating rate $p$. The total communication costs are $\{0, 60, 100, 150, 200, 250\}$.}
		\label{fig:probfull}
	\end{minipage}
	\begin{minipage}[t]{1\textwidth}
		\centering
		\includegraphics[width=12cm]{../figures/R_full}
		\caption{Regrets of CDP-MAB with limited communication rounds $R$. The total communication costs are $\{50, 100, 150, 200, 250, 300\}$. }
			\label{fig:rfull}
	\end{minipage}
\end{figure}


\subsubsection{Effect of User Participating Rate $p$}
We then fix the privacy-preserving level as $\epsilon = 0.5$ and discuss the effect of communication-reduction strategies. In particular, we consider 5  different participating rates $p = \{0.02,0.2,0.4,0.6,0.8,1\}$. Among that, $p=0.02$ indicates the no communication case where each agent select actions only based on the local observations. $p=1$ indicates the fully participating case that all agents send their perturbed models to the server after each epoch.  Other choices of $p$ indicate that only part of the agents participate in the communication. Figure. \ref{fig:probfull} shows that the regrets at $T$ decrease as $p$ increases.

%\begin{figure}[h]
	%\centering
	%\includegraphics[width=0.7\linewidth]{../figures/prob_full}
	%\caption{regrets of CDP-MAB with different participating rate $p$.}
%	\label{fig:probfull}
%\end{figure}


\subsubsection{Effect of  Limited Communication Rounds $R$}
In this part, we fix both privacy level as $\epsilon = 0.5$ and participating rate as $p=1$, and show the effect of the communication rounds constraints. We consider the number of communication rounds $R$ varying in $\{1,2,3,4,5,6\}$. Fr0m Table \ref{tab:round}, we can see that our algorithm can correctly identify the optimal arm after the last communication round, and exploit it until time $T$. However, $R=1$ indicates the case that we have distinct one exploration phase and one exploitation phase. That is, We must eliminate all suboptimal arms after epoch 1 with a high probability. Figure. \ref {fig:rfull} shows that the regrets decrease with $R$ increase. It is worth noting that the regret we reached at $ R=5$ and 6 are almost the same. This is because in the randomly generated instance, $\Delta=0.0109$, which indicates that we need about $ \log(1/\Delta) \approx 5$. When $R>5$, the term $\Delta^{R/2}$ in Thereon 2 tends to a constant and do not affect the total regrets. 
\begin{table}[htbp]
\centering
	\caption{Remaining arms after each communication round}
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		& Epoch =1   & Epoch =2            & Epoch = 3        & Epoch = 4     & Epoch = 5 \\ \hline
		R = 1 & All $K$ arms & [23]           & -                & -             & -         \\ \hline
		R = 2 & All $K$ arms & [3,23,28,43]  & [23]        & -             & -         \\ \hline
		R = 3 & All $K$ arms & [3, 8, 16, 17, 23, 24, 28, 29, 43] &  [3,23,28,43]& [23]    & -         \\ \hline
		R = 4 & All $K$ arms & [3, 7, 8, 16, 17, 23, 24, 26, 27, 28, 29, 43, 45] &  [3,23,28,43]&  [3,23,43] & [23] \\ \hline
	\end{tabular}
	
	\label{tab:round}
\end{table}

%\begin{figure}[h]
	%\centering
	%\includegraphics[width=0.7\linewidth]{../figures/R_full}
	%\caption{regrets of CDP-MAB with limited communication rounds $R$.}
	%\label{fig:rfull}
%\end{figure}

\subsubsection{Combination of $p$ and $R$}

We finally combine these two communication constraints $p$ and $R$ with privacy parameter $\epsilon = 1$. With different pairs of $(p,R)$, we compare the final cumulative regret $R_{Alg1}(T)$ achieved at time slot $T$ as well as the total communication cost $C_{Alg1}(T)$. Fig.~\ref{fig:combpr} shows a clear trade-off between the communication cost and learning performance. Note that $R=5,p=1$ is close to the largest amount of required communication cost of the centralized setting. Correspondingly, the regret of this case is close to the performance in Fig. \ref{fig:epsilon} with $\epsilon = 1$.
%\begin{figure}[h]
%	\centering
	%\includegraphics[width=0.6\linewidth]{../figures/comb_pr}
	%\caption{Regrets  of CDP-MAB with communication constraints $p$ and  $R$.}
%	\label{fig:combpr}
%\end{figure}
\vspace{-0.8cm}
\begin{figure}[htbp]
	\centering
	\begin{minipage}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=7.5cm]{../figures/comb_pr}
		\caption{Regrets of CDP-MAB with participate rate $p$ and communication rounds $R$.}
		\label{fig:combpr}
	\end{minipage}
	\begin{minipage}[t]{0.48\textwidth}
		\centering
		\includegraphics[width=7.5cm]{../figures/comb_pd}
		\caption{Regrets of DDP-MAB with $d$-regular graph and link connection probability $p$.}
		\label{fig:combpd}
	\end{minipage}
\end{figure}

\subsection{Decentralized setting}
In this part we investigate how the properties of graphs can effect the learning performance in the decentralized setting.
\subsubsection{Effect of  Network Structure}
 We first fix the link connection probability as $p = 1$ and consider 4 different $d$-regular graph with $d = \{2,5,10,20,49\}$. Here the graph with $d=2$ can be seen as the cycle-graph and $d=49$ is the fully-connected graph. The communication cost of each choice of d is $\{250, 500,750,1000,1225\}$. Fig. \ref{fig:d}  shows the large $d$ results in less regret. We can see that when $d = M-1 = 49$, we  achieve a total regret of around $5\times 10^4$, which is consistent to the best performance we reach in the centralized setting. However, with the server, we only need 250 communication cost. 



\begin{figure}[htbp]
	\begin{minipage}[t]{0.45\textwidth}

		\includegraphics[width=7.5cm]{../figures/d}
		\caption{Regrets  of DDP-MAB with different $d$-regular graph. The total communication costs are $\{1250,2500,3750,6000,6125\}$.}
		\label{fig:d}
	\end{minipage}\hspace{5mm}
	\begin{minipage}[t]{0.45\textwidth}
		\includegraphics[width=7.5cm]{../figures/dp}
		\caption{Regrets  of DDP-MAB with different link connection probability $p$. The total communication costs are $\{1200,2000,3000,4000,5000\}$.}
		\label{fig:dp}
	\end{minipage}\hspace{5mm}
\end{figure}

%\begin{figure}
	%\centering
%	\includegraphics[width=0.7\linewidth]{../figures/d}
	%\caption{}
%	\label{fig:d}
%\end{figure}


\subsubsection{Effect of  Link Connection Probability}
We then consider the effect of link connection probability $p$ on a special $40$- regular graph. We set $p$ varying in $\{0.2,0.4,0.6,0.8,1\}$ to represent the probability that each agent can receive the messages from its neighbors. The communication cost of each choice of $p$ is $\{150, 300, 450, 600, 750\}$. Fig. \ref{fig:dp} shows the similar trade-off in Fig. \ref{fig:d}. Besides, comparing with the two figures, we can obtain the same results, for example, $d=20, p=1$ has a smaller regret than $d=40,p=0.4$. To better show the performance of different pair $(p,d)$, we compare the cumulative regret $R_{Alg2}(T)$ achieved at time slot $T$ as well as the total communication cost $C_{Alg2}(T)$, as shown in Fig. \ref{fig:combpd}. From Fig. \ref{fig:combpd}, we can see a clear trade-off between communication cost and learning performance. Beside, compared with Fig. \ref{fig:combpr}, larger communication cost is needed if we want to achieve similar regret as in the centralized setting.

%\begin{figure}
	%\centering
	%\includegraphics[width=0.7\linewidth]{../figures/dp}
%	\caption{}
%	\label{fig:dp}
%\end{figure}


%\begin{figure}
%	\centering
	%\includegraphics[width=0.6\linewidth]{../figures/comb_pd}
%	\caption{Regrets of DDP-MAB with $p$ and $d$.}
%\label{fig:combpd}
%\end{figure}

\subsection{Hybrid setting}
In this section, we divide 50 agents into $Q = 5$ components with different properties. We list $M_q, p_q, d_q$ of each component $q$ and corresponding $p_c$ in Table \ref{tab:hybrid}. %We pay more attention to the per-agent regret in different component rather than the total regret in this section.

\begin{table}[h]
	\centering
		\caption{Different settings for hybrid structure}
	\begin{tabular}{|c|c|c|c|c|}
		\hline
		& $\{M_q \}$                & $\{p_q \} $                 & $\{d_q \} $        & $p_c$ \\ \hline
		case 1 & {[}10,10,10,10,10{]} & {[}1,1,1,1,1{]}         & $M_q$-1          & 1    \\ \hline
		case 3 & {[}10,10,10,10,10{]} & {[}1,1,1,1,1{]}         & $M_q$-1          & 0.5  \\ \hline
		case 3 & {[}10,10,10,10,10{]} & {[}1,1,1,1,1{]}         & $M_q$-1          & 0.2  \\ \hline
		case 4 & {[}10,10,10,10,10{]} & {[}0.2,0.4,0.6,0.8,1{]} & $M_q$-1          & 1    \\ \hline
		case 5 & {[}10,10,10,10,10{]} & {[}1,1,1,1,1{]}         & [2,4,6,8,9] & 1    \\ \hline
		case 6 & {[}25,10,5,3,2{]}    & {[}1,1,1,1,1{]}         & $M_q$-1          & 1    \\ \hline
	\end{tabular}

	\label{tab:hybrid}
\end{table}



\begin{figure}[htbp]
\centering
\subfigure[Per-agent regrets of HDP-MAB with different $p_c$.]{
	\begin{minipage}{0.48\textwidth}
		\centering
		\includegraphics[width=7cm]{../figures/case123}
		\label{fig:case123}
		%\caption{Per-agent regrets of HDP-MAB with different $p_c$.}
	\end{minipage}%
}%
\subfigure[Per-agent regrets of HDP-MAB with different $p_q$.]{
	\begin{minipage}{0.48\textwidth}
		\centering
		\includegraphics[width=7.5cm]{../figures/case4}
		\label{fig:case4}
		%\caption{Per-agent regrets of HDP-MAB with different $p_c$.}
	\end{minipage}
}
\subfigure[Per-agent regrets of HDP-MAB with different $d_q$.]{
	\begin{minipage}{0.48\textwidth}
		\centering
		\includegraphics[width=7.5cm]{../figures/case5}
		\label{fig:case5}
		%\caption{Per-agent regrets of HDP-MAB with different $p_c$.}
	\end{minipage}%
}%
\subfigure[Per-agent regrets of HDP-MAB with different $M_q$.]{
	\begin{minipage}{0.48\textwidth}
		\centering
		\includegraphics[width=7.5cm]{../figures/case6}
		\label{fig:case6}
		%caption{Per-agent learning regrets of HDP-MAB with different $p_c$.}
	\end{minipage}
}
\caption{Per-agent regrets of HDP-MAB.}
\end{figure}


\subsubsection{Effect of Component Participating Rate $p_c$}
In case 1, 2, 3, we assign $M_q = 10$ agents in each components, which are fully connected ($p_q = 1,  d_q = M_q -1$). According to our Alg. 3, components with the same structure will bring similar per-agent regret. So we only need to consider the impact of $p_c$. In case 3, $p_c = 0.2 = 1/Q$ indicates that the agent only exchanges messages inside the component, without the knowledge of other components. In case 1, $p_c = 1$ indicates that each component sends the local aggregation information to the server at each communication round. Fig. \ref{fig:case123} shows that the per-agent regret increases as the communication cost ($p_c$) decreases as they need to perform more intra-component exploration without the knowledge of other components. We also notice that when $p_c = 1$, the total regret over all $M$ agents is $5\times 10^4$, which is the best performance the CDP-MAB can achieve with $p=1$ and DDP-MAB can achieve with $d=M-1$ and $p=1$. The communication costs of these two best case are $250$ and $6125$. The HDP-MAB achieve $275$ communication cost.  This also matches with the results that we directly obtain from Theorem 4 in Fig. 3.


\subsubsection{Effect of Network structure of Each Component}
We then fix $p_c = 1$ and change the structure of each component. We choose $p_q=\{0.2,0.4,0.6,0.8,1\}$ and $d_q = \{1,3,5,7,9\}$ for component $q = 1$ to 5. The per-agent regret and corresponding communication cost are shown in Fig.  \ref{fig:case4} and Fig.   \ref{fig:case5}. We can see that the well-connected component leads to smaller per-agent regret, since they can use a less number of samples to achieve the required number of observations. 

\subsubsection{Effect of Number of Agents in Each Component}
We finally consider the effect of the number of agents inside each components. This case is more practical to simulate the IoT application, where the each household is equipped with different number of smart devices. We set $M_q = {25,10,5,3,2}$ for  component $q = 1$ to 5. The results in Fig. \ref{fig:case6} shows that the component with a large $M_q$ reaches a smaller per-agent regret and larger communication cost. %This is because they can reduce the sample with the help of their connected neighbors. 





\section{Conclusion}

In this paper, we propose a privacy-preserving communication-efficient framework to tackle the privacy leakage and large communication overhead issues in the FMAB problem. To protect the user privacy, we use DP techniques by adding noise before the agents send their local parameters. Theoretical results show that the DP mechanism brings a $\frac{1}{\epsilon}$ trade-off between privacy and utility.  Partial participation and less frequent communication strategies are utilized to reduce the communication cost. In the centralized setting, our CDP-MAB algorithm with partial participation rate $p$ and limited communication rounds $R$ achieves a regret of $(\frac{\Delta^{-2/R} K \log T}{p\min\{\epsilon,\Delta\}})$ with a communication cost of $pMR$. In the decentralized setting, we consider a $d$-regular graph with connection probability $p$ as a special case. Our proposed DDP-MAB algorithm achieves a $O(\frac{M\Delta^{-2/R}\log T}{(1+pd)\min\{\epsilon,\Delta\}})$ regret with a  $\frac{pdMR}{2}$ communication cost. We finally propose the HDP-MAB algorithm, where each component is a connected graph and can communicate with other components through the server. Results show that, the component with more agents and strong connections can achieve a smaller per-agent regret. We finally verified the above theoretical results by conducting extensive experiments.
\section*{Acknowledgement}
We would like to thank  Prof. Christina Fragouli from UCLA for her valuable discussions and  insightful comments when we were conducting this work.


